FLUXLAYER: High-Performance Design for Cross-chain Fragmented Liquidity

Autonomous Market Makers (AMMs) rely on arbitrage to facilitate passive price updates. Liquidity fragmentation poses a complex challenge across different blockchain networks. This paper proposes FluxLayer, a solution to mitigate fragmented liquidity and capture the maximum extractable value (MEV) in a cross-chain environment. FluxLayer is a three-layer framework that integrates a settlement layer, an intent layer, and an under-collateralised leverage lending vault mechanism. Our evaluation demonstrates that FluxLayer can effectively enhance cross-chain MEV by capturing more arbitrage opportunities, reducing costs, and improving overall liquidity.

==> packed/swap.tex <==
\begin{figure}[t]
    % Subfigure 1: Cross-chain Quote
    \subfigure[Cross-chain Quote]{  
        \label{fig:cross-chain-quote}
        \begin{minipage}{\linewidth} % Ensure both subfigures take equal width
            \begin{tikzpicture}
            \begin{axis}[
                width=1\linewidth, height=6cm, % Full width of minipage
                ymin=0, ymax=1000,
                ymajorgrids=true,
                x tick label style={rotate=45, anchor=east, font=\scriptsize}, 
                symbolic x coords={
                    0.001, 0.0012, 0.0013, 0.0014, 0.0015, 
                    0.01, 0.012, 0.013, 0.014, 0.015,
                    0.05, 0.052, 0.053, 0.054, 0.055,
                    0.1, 0.12, 0.13, 0.14, 0.15,
                    0.5, 0.52, 0.53
                },
                xtick=data,
                legend style={at={(0.5,1.2)}, anchor=north, legend columns=-1, font=\scriptsize},
                ylabel={Value}, ylabel style={font=\scriptsize},
                xlabel={BTC}, xlabel style={font=\scriptsize},
                tick label style={font=\scriptsize}
            ]

            % Slippage
            \addplot[
                color=cyan, thick, mark=*,
                mark size=1.5pt, mark options={solid, fill=cyan}
            ]
            coordinates {
                (0.001, 500)
                (0.0012, 578)
                (0.0013, 578)
                (0.0014, 919)
                (0.0015, 919)
                (0.01, 181)
                (0.012, 500)
                (0.013, 181)
                (0.014, 104)
                (0.015, 111)
                (0.05, 500)
                (0.052, 169)
                (0.053, 64)
                (0.054, 169)
                (0.055, 132)
                (0.1, 7.5)
                (0.12, 167)
                (0.13, 59)
                (0.14, 167)
                (0.15, 200)
                (0.5, 173)
                (0.52, 173)
                (0.53, 100)
            };
            \addlegendentry{Slippage}

            % Revenue
            \addplot[
                color=green, thick, mark=*,
                mark size=1.5pt, mark options={solid, fill=green}
            ]
            coordinates {
                (0.001, 3.99)
                (0.0012, 5.15)
                (0.0013, 5.15)
                (0.0014, 9.44)
                (0.0015, 9.44)
                (0.01, 3.48)
                (0.012, 3.6)
                (0.013, 5.56)
                (0.014, 7.88)
                (0.015, 9.28)
                (0.05, 6.33)
                (0.052, 13.69)
                (0.053, 18.5)
                (0.054, 40.86)
                (0.055, 83.2)
                (0.1, 9.76)
                (0.12, 29.4)
                (0.13, 29.98)
                (0.14, 127.68)
                (0.15, 295.97)
                (0.5, 123.92)
                (0.52, 355.79)
                (0.53, 367.48)
            };
            \addlegendentry{Revenue}
            \end{axis}
            \end{tikzpicture}
        \end{minipage}
    }
    \hfill
    % Subfigure 2: Cross-chain Swap
    \subfigure[Cross-chain Swap]{\label{fig:cross-chain-swap}
        \begin{minipage}{\linewidth}
            \begin{tikzpicture}
            \begin{axis}[
                width=1\linewidth, height=6cm, % Ensure consistent dimensions
                ymajorgrids, xmajorgrids, grid style=dashed,
                xlabel style={font=\scriptsize}, ylabel style={font=\scriptsize},
                legend style={
                    at={(0.5,1.2)}, anchor=north, legend columns=-1, font=\scriptsize
                },
                symbolic x coords={
                    0.002, 0.013, 0.016, 0.021, 0.027, 0.027, 0.029, 0.032, 0.032, 0.034, 0.035, 0.041, 0.183, 0.500, 0.781, 0.853, 1.069, 1.388, 1.870, 1.999, 2.971
                },
                xtick=data,
                x tick label style={rotate=45, anchor=east, font=\scriptsize}, 
                ylabel={Values}, xlabel={BTC}, ymin=0, ymax=1400
            ]

            % Revenue
            \addplot+[mark=o, color=cyan] coordinates {
(0.002, 0.32)
(0.013, 6.98)
(0.016, 35.64)
(0.021, 6.85)
(0.027, 19.46)
(0.027, 17.19)
(0.029, 10.04)
(0.032, 13.65)
(0.032, 21.89)
(0.034, 5.91)
(0.035, 14.42)
(0.041, 29.97)
(0.183, 1305.27)
(0.500, 357.50)
(0.781, 122.34)
(0.853, 93.96)
(1.069, 246.19)
(1.388, 133.07)
(1.870, 192.49)
(1.999, 186.30)
(2.971, 1073.60)
            };
            \addlegendentry{Revenue}

            % Time
            \addplot+[mark=triangle*, color=green] coordinates {
                (0.002,18)
(0.013,135)
(0.016,900)
(0.021,1200)
(0.027,900)
(0.027,900)
(0.029,120)
(0.032,1200)
(0.032,1200)
(0.034,600)
(0.035,126)
(0.041,180)
(0.183,1200)
(0.500,900)
(0.781,600)
(0.853,1200)
(1.069,600)
(1.388,600)
(1.870,1200)
(1.999,1200)
(2.971,1200)
            };
            \addlegendentry{Time (Seconds)}
            \end{axis}
            \end{tikzpicture}
        \end{minipage}
    }

    \caption{\textbf{Cross-chain Inquiries} }
    \label{fig:cross-chain}
\end{figure}

